Image Search with Text Feedback by Additive Attention Compositional Learning

Effective image retrieval with text feedback stands to impact a range of real-world applications, such as e-commerce. Given a source image and text feedback that describes the desired modifications to that image, the goal is to retrieve the target images that resemble the source yet satisfy the given modifications by composing a multi-modal (image-text) query. We propose a novel solution to this problem, Additive Attention Compositional Learning (AACL), that uses a multi-modal transformer-based architecture and effectively models the image-text contexts. Specifically, we propose a novel image-text composition module based on additive attention that can be seamlessly plugged into deep neural networks. We also introduce a new challenging benchmark derived from the Shopping100k dataset. AACL is evaluated on three large-scale datasets (FashionIQ, Fashion200k, and Shopping100k), each with strong baselines. Extensive experiments show that AACL achieves new state-of-the-art results on all three datasets.

==> latex/tables/ablation_attention.tex <==
\renewcommand{\tabcolsep}{2pt}

\begin{table}[ht]
\centering
% \setlength{\abovecaptionskip}{-0.05pt}
% \setlength{\belowcaptionskip}{-0.4cm} 

\resizebox{\linewidth}{!}{
\begin{tabular}{l|ll|ll|ll}
\multirow{2}{*}{Method}         & \multicolumn{2}{|c|}{Shirt}     & \multicolumn{2}{c|}{Dress}    & \multicolumn{2}{c}{Toptee}          \\ \cline{2-7} 
               & \multicolumn{1}{|c}{R@10}       & \multicolumn{1}{c|}{R@50}     & \multicolumn{1}{c}{R@10} & \multicolumn{1}{c|}{R@50} & \multicolumn{1}{c}{R@10} & \multicolumn{1}{c}{R@50} \\ 
\toprule

Dot-product & \multicolumn{1}{|c}{±} & \multicolumn{1}{c|}{±}  & \multicolumn{1}{c}{±}  & \multicolumn{1}{c|}{±}   & \multicolumn{1}{c}{±}   &  \multicolumn{1}{c}{±}   \\

\end{tabular}}
\caption{Ablation study on Additive Self-Attention.}
\label{tab:ablation_interact}
\end{table}

==> latex/tables/ablation_fast.tex <==
\renewcommand{\tabcolsep}{6pt}

\begin{table}[t]
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{l|ll|ll|ll}
\multirow{2}{*}{Stage(s)}
             & \multicolumn{2}{|c|}{Shirt}     & \multicolumn{2}{c|}{Dress}    & \multicolumn{2}{c}{Toptee}  \\ 
\cline{2-7} 
               & \multicolumn{1}{|c}{R@10}       & \multicolumn{1}{c|}{R@50}     & \multicolumn{1}{c}{R@10} & \multicolumn{1}{c|}{R@50} & \multicolumn{1}{c}{R@10} & \multicolumn{1}{c}{R@50} \\ 
\toprule
Stage 2+3+4 & \multicolumn{1}{|c}{22.09} & \multicolumn{1}{c|}{46.24}  & \multicolumn{1}{c}{27.87}  & \multicolumn{1}{c|}{54.03}   & \multicolumn{1}{c}{28.24}   &  \multicolumn{1}{c}{55.06}    \\

Stage 3+4  &\multicolumn{1}{|c}{\textbf{24.82}} & \multicolumn{1}{c|}{\textbf{48.85}}  & \multicolumn{1}{c}{\textbf{29.89}}  & \multicolumn{1}{c|}{\textbf{55.85}}   & \multicolumn{1}{c}{\textbf{30.88}}   &  \multicolumn{1}{c}{\textbf{56.85}} \\
Stage 4   &\multicolumn{1}{|c}{23.66} & \multicolumn{1}{c|}{48.32}  & \multicolumn{1}{c}{28.84}  & \multicolumn{1}{c|}{55.03}   & \multicolumn{1}{c}{28.64}   &  \multicolumn{1}{c}{56.39}  \\

% Stage 2+3+4 & \multicolumn{1}{|c}{22.09±0.62} & \multicolumn{1}{c|}{46.24±1.04}  & \multicolumn{1}{c}{27.87±0.28}  & \multicolumn{1}{c|}{54.03±0.17}   & \multicolumn{1}{c}{28.24±0.90}   &  \multicolumn{1}{c}{55.06±0.33}    \\

% Stage 3+4  &\multicolumn{1}{|c}{\textbf{24.82±0.62}} & \multicolumn{1}{c|}{\textbf{48.85±0.77}}  & \multicolumn{1}{c}{\textbf{29.89±0.65}}  & \multicolumn{1}{c|}{\textbf{55.85±0.87}}   & \multicolumn{1}{c}{\textbf{30.88±1.2}}   &  \multicolumn{1}{c}{\textbf{56.85±1.16}} \\
% Stage 4   &\multicolumn{1}{|c}{23.66±1.39} & \multicolumn{1}{c|}{48.32±1.56}  & \multicolumn{1}{c}{28.84±1.79}  & \multicolumn{1}{c|}{55.03±1.72}   & \multicolumn{1}{c}{28.64±1.77}   &  \multicolumn{1}{c}{56.39±1.98}  \\


\end{tabular}}
\caption{Ablation of using tokens from different Swin Transformer stages on FashionIQ dataset.}
\label{tab:ablation}
\end{table}

==> latex/tables/ablation_interact.tex <==
\renewcommand{\tabcolsep}{6pt}

\begin{table}[ht]
\centering
% \setlength{\abovecaptionskip}{-0.05pt}
% \setlength{\belowcaptionskip}{-0.4cm} 

\resizebox{\linewidth}{!}{
\begin{tabular}{l|ll|ll|ll}
\multirow{2}{*}{Method}         & \multicolumn{2}{|c|}{Shirt}     & \multicolumn{2}{c|}{Dress}    & \multicolumn{2}{c}{Toptee}          \\ \cline{2-7} 
               & \multicolumn{1}{|c}{R@10}       & \multicolumn{1}{c|}{R@50}     & \multicolumn{1}{c}{R@10} & \multicolumn{1}{c|}{R@50} & \multicolumn{1}{c}{R@10} & \multicolumn{1}{c}{R@50} \\ 
\toprule
% Additive$\rightarrow$Dot-Product & \multicolumn{1}{|c}{24.88} & \multicolumn{1}{c|}{48.31}  & \multicolumn{1}{c}{29.49}  & \multicolumn{1}{c|}{54.70}   & \multicolumn{1}{c}{29.64}   &  \multicolumn{1}{c}{55.53}   \\

Addition & \multicolumn{1}{|c}{24.71} & \multicolumn{1}{c|}{48.35}  & \multicolumn{1}{c}{28.80}  & \multicolumn{1}{c|}{54.74}   & \multicolumn{1}{c}{29.30}   &  \multicolumn{1}{c}{56.56}   \\

Product  &\multicolumn{1}{|c}{\textbf{24.82}} & \multicolumn{1}{c|}{\textbf{48.85}}  & \multicolumn{1}{c}{\textbf{29.89}}  & \multicolumn{1}{c|}{\textbf{55.85}}   & \multicolumn{1}{c}{\textbf{30.88}}   &  \multicolumn{1}{c}{\textbf{56.85}}   \\ 

\end{tabular}}
\caption{Ablation of interaction function on FashionIQ dataset.} 
% Additive$\rightarrow$Dot-Product: substituting the additive self-attention layer with a standard dot-product one. 
% Product$\rightarrow$Addition:change the Hadamard product to addition.}
\label{tab:ablation_interact}
\end{table}

==> latex/tables/shop100k_stage.tex <==
\renewcommand{\tabcolsep}{11pt}

\begin{table}[t]
% \setlength{\abovecaptionskip}{-0.2cm} 
% \setlength{\belowcaptionskip}{-0.3cm} 

\centering
\resizebox{0.5\linewidth}{!}{
\begin{tabular}{l|ccc}
{Stage(s)} &Recall@1  &Recall@10 &Recall@50\\ 
\toprule
Stage 2 + 3 + 4 & 11.92 & 48.78 & 80.74\\
Stage 3 + 4  & \textbf{12.26}  & \textbf{49.20}  & \textbf{81.29}\\
Stage 4    & 12.01  & 48.56  & 81.25\\

\end{tabular}}
\caption{Ablation of using tokens from different Swin Transformer stages on our modified Shopping100k dataset.}
\label{tab:shop100kstage}
\end{table}
